A Game-Theoretic Approach to Self-Stabilization with Selfish Agents

Self-stabilization is an excellent approach for adding fault tolerance to a distributed multi-agent system. However, two properties of self-stabilization theory, convergence and closure, may not be satisfied if agents are selfish. To guarantee convergence, we formulate the problem as a stochastic Bayesian game and introduce probabilistic self-stabilization to adjust the probabilities of rules with behavior strategies. This satisfies agents' self-interests such that no agent deviates the rules. To guarantee closure in the presence of selfish agents, we propose fault-containment as a method to constrain legitimate configurations of the self-stabilizing system to be Nash equilibria. We also assume selfish agents as capable of performing unauthorized actions at any time, which threatens both properties, and present a stepwise solution to handle it. As a case study, we consider the problem of distributed clustering and propose five self-stabilizing algorithms for forming clusters. Simulation results show that our algorithms react correctly to rule deviations and outperform comparable schemes in terms of fairness and stabilization time.

==> model.tex <==
%%!TEX PS-program = pdflatexmk
%%!TEX root = newpaper.tex

\section{Game Theoretic Approach}
\label{section:model}

In this section, we present a game theoretic approach for studying self-stabilizing MASs. This will allow us to design mixed strategies %associated with the probabilistic rules of an algorithm 
that tolerate selfish behavior.


Game theory is a natural framework for modeling self-stabilizing systems wherein players alternate their actions in each configuration and the game is repeated many times until the system terminates in a legitimate configuration. Considering that a distributed scheduler is defined by a probability distribution that depends on the latest actions and the current configuration, a game that models a distributed self-stabilizing system is a stochastic game \cite{shapley_stochastic_1953}, i.e., a dynamic game with probabilistic transitions.


%A Stochastic game, introduced by Shapley \cite{shapley_stochastic_1953}, models dynamic interactions, where the environment changes in response to agent behavior. We can view it as an expansion of a Markov decision process (MDP) where there are multiple agents with possibly conflicting goals, and the actions taken by all agents determine state transitions and rewards (payoffs) \cite{solan_stochastic_2015}. It is also a generalization of repeated games where the game played at any stage depends on the previous game and on the joint actions of agents in that game. \dt{This is tutorial and not needed}

A stochastic game is a tuple $\left<V,S,\{A_v^s\}, T,\delta,s^0,\{U_v^s\}\right>$ \cite{solan_discounted_1998}, where
\begin{itemize}
	\item $V$ is a finite set of agents indexed $1,\dots,n$,
	\item $S$ is a finite set of states,
	\item $A_v^s$ is a set of actions available to agent $v$ in state $s$,
	\item $T$ is a distribution on the state space $S$, where $T(s'\mid s, \vec{a})$ denotes the probability that the system transitions to state $s'$ given joint action $\vec{a} \in \prod_{v\in V}A_v^s$ is performed in state $s$,
	\item $\delta$ is a discount factor, where $0<\delta\le1$,
	\item $s^0$ is an initial state,
	\item $U_v^s(\vec{a})$ is a payoff function for agent $v$, state $s$, and joint action $\vec{a}$.
\end{itemize}

The game starts in state $s^0$. At each stage $t$, all agents concurrently choose actions $a_v$ from the possible pure actions given by the set $A_v^s$. This generates payoffs $\{U_v^s(\vec{a})\}_v$ and the next state is chosen according to $T$. Agents discount their future payoffs based on the discount factor $\delta$ .

The equilibrium concept to a stochastic game is Markov perfect equilibrium \cite{maskin_markov_2001}, analogous to subgame perfect equilibrium for extensive form games. A strategy that only depends on the current state not the history is called Markov strategy.
%\dt{I don't understand - rephrase.}
Markov perfect equilibrium is a strategy profile consisting of only Markov strategies that is a Nash equilibrium regardless of the starting state.

Note that if the probabilistic self-stabilizing algorithm is designed correctly in response to the agent preferences, we expect the system to eventually converge to a legitimate configuration and to maintain a legitimate configuration thereafter. Also, because of the rationality constraint imposed on unilateral deviations in a legitimate configuration, assuming that no legitimate configuration can be reached from another through a unilateral move, no agent will make a move while in a legitimate configuration. Therefore, the corresponding game has a finite number of stages
%\dt{steps?}
 and we do not need to assume agents discount the future.

%If a self-stabilizing system is completely observable (not locally) \dt{ what does this mean?  Have you defined earlier?}, a stochastic game-theoretic approach suffice to model the game among agents; otherwise, we have to address uncertainty as a result of a) a partially observable environment, and/or b) incomplete information about the system graph. \dt{Is this an example of a partially observed environment?}

%Unless otherwise specified, a stochastic game assumes agents have complete information about the state of the game; in this respect, a stochastic game generalizes work on completely observable MDPs \cite{yamamoto_stochastic_2019}. Neither MASs nor distributed computing systems satisfy this assumption. Partially observable problems, those in which agents do not have full access to the world state at every stage, are prevalent in MASs where agents have limited and noisy connectivity.

A stochastic game assumes agents have complete information about the state of the game; in this respect, a stochastic game generalizes work on completely observable MDPs \cite{yamamoto_stochastic_2019}; however, unless otherwise specified, neither MASs nor distributed computing systems satisfy this assumption. Partially observable problems, those in which agents do not have full access to the world state at every stage, are prevalent in MASs where agents have limited and noisy connectivity. Therefore, a stochastic game-theoretic approach does not suffice to model the game among agents in a self-stabilizing systems and we have to address uncertainty as a result of a) a partially observable configuration (i.e. the states of all agents), and/or b) incomplete information about the system graph.

Partially observable Markov decision processes (POMDPs) have been successfully applied to single-agent problems; however, this framework does not generalize well to the distributed MASs. All agents would have to maintain parallel POMDPs representing the system's joint belief state, taking all other agent observations as input. Not only does this algorithm scale exponentially with the number of agents and observations, but it also requires unlimited bandwidth and instantaneous communication between the agents while in a wide range of real-world scenarios, agents are limited to low bandwidth connection on a single channel. If no communication is available, this approach is no longer correct: each agent will acquire different observations, leading to different belief states that cannot be reconciled. Therefore, we agents with limited knowledge of other agents' observations must reason about all possible belief states that could be held by other agents and how that affects their own action selection \cite{wray_distributed_nodate,emery2004approximate}.

Partially Observable Stochastic Games (POSGs) is a game theoretic approach to multi-agent decision making in partial observable environments that implicitly models a distribution over other agent belief states. A POSG is a tuple $\left<V,S,\{A_v^s\},\{O_v\},T,\delta,{b_v^0},\{U_v^s\}\right>$, where
\begin{itemize}
	\item $V$, $S$, $\{A_v^s\}$, $\delta$, and $\{U_v^s\}$ are similar to their counterparts in a stochastic game,
	\item $O_v$ is a finite set of observations for agent $v$,
	\item $T$ is a distribution on the state space $S$ and joint observations $\prod_{v\in V}O_v$, where, given joint action$\vec{a}$ is performed in state $s$, $T(s',\vec{o}\mid s, \vec{a})$ denotes the probability the system transitions to state $s$ and generates observation j$\vec{o}$,
	\item $b_v^0 \in \Delta(S)$ is the initial belief of agent $v$ over states.
\end{itemize}

Agents choose their actions by solving the POSG to find a policy $\sigma_v$ for each agent that defines a probability distribution over the actions it should take at each stage. A dynamic programming algorithm for POSGs is proposed in \cite{hansen_dynamic_nodate}, which is a synthesis of dynamic programming for POMDPs and iterated elimination of dominated strategies in normal form games.

An agent in a self-stabilizing MAS, as well as a process in a distributed system, normally updates its primary variables in every stage based on the observable information in that stage \cite{jaggard_dynamics_2017}. Let $\lambda_v$ denote a local state of agent $v$, i.e, the primary variables of $v$ and other agents that $v$ directly interacts with; and let $\Lambda_v$ denote a finite set of all local states of $v$. Let $\ell_v$ denote the neighborhood of agent $v$ (including itself). Let $o_v$ be an observation for agent $v$, i.e., a temporary record of variables located at $\ell_v$ collected via message passing. When communications are fully synchronized and reliable, $\lambda_v$ is accurately extracted from $o_v$; otherwise, we need to estimate $\lambda_v$ from $o_v$. 

Let $C$ denote the set of all configurations of a self-stabilizing MAS; they correspond to the set of states in the game. Given gain function $g_v(c)$ and transition probability given action $\vec{a}$, $\Pr(c'\mid c,\vec{a})$ for all $c,c'\in C$, the payoff of agent $v$ after joint actions $\vec{a}$ in configuration $c$ is
\begin{equation}
\label{x4_eq}
U_v^c(\vec{a})=\sum_{c'\in C}\Pr(c'\mid c,\vec{a})\big(g_v(c')-g_v(c)\big)
\end{equation}
Let $T(c',\vec{o}\mid c, \vec{a})$ denote the probability of transiting to configuration $c'$ and generating  joint observation $\vec{o}=\left<o_1,\dots,o_{|V|}\right>$ from configuration $c$ after executing $\vec{a}$ . Given that $\vec{o}$ depends on the new configuration $c'$ and on the just taken joint action $\vec{a}$ with probability $\Pr(\vec{o}\mid c',\vec{a})$, we have
\begin{equation}
\label{xxxx_eq}
T(c',\vec{o}\mid c,\vec{a})=\Pr(c'\mid c,\vec{a})\Pr(\vec{o}\mid c',\vec{a})
\end{equation}
Because an agent does not observe the global state, it must make decisions under uncertainty of the true configuration. However, by communicating with the system and receiving observations about its local state, the agent may update its belief (i.e., a description of the uncertainty) in the true configuration by updating the probability distribution of the current configuration. Nevertheless, given that the graph representing the system is known, because the observations of an agent are limited to its neighborhood, an agent estimates the current configuration from the observed local state and its belief in the states of agents beyond the boundaries of its neighborhood. %only depends on the initial belief, unless the observations are public, \dt{ppublic?} which contradicts the distributed nature of a self-stabilizing MAS. \dt{You started using the term ``belief''.  What does that mean?}

Given that the configuration is Markovian, after having taken joint action $\vec{a}$ and observing $o_v$, agent $v$ solely requires knowledge of its previous belief, the joint actions
 %\dt{can an agent know all joint actions?}
 taken, and its current observation to update its belief over configurations. We can denote this by a function, call it $\tau$, where $b'_v=\tau(b_v,\vec{a},o_v)$.
 
 Let $b_v(c)$ denote the belief agent $v$ has that the current configuration is $c$. Given $\Pr(o_v\mid c',\vec{a})$ and $\Pr(c'\mid c,\vec{a})$, we have
\begin{equation}
\label{xxx_eq}
b_v'(c')=\frac{\Pr(o_v\mid c',\vec{a})\sum _{{c\in C}}\Pr(c'\mid c,\vec{a})b(c)}{\sum_{{c'\in C}}\Pr(o_v\mid c',\vec{a})\sum _{{c\in C}}\Pr(c'\mid c,\vec{a})b(c)}.
%b^{\vec{a},o_v}(c)=\sum_{\lambda_v\in \Lambda_v}\Pr(c\mid \lambda_v)\Pr(\lambda_v\mid o_v,\vec{a})
\end{equation}

%One major problem with POSG (and also SG) arises when the assumption that agents know $V$ and $C$, is invalid.  Unfortunately, this is often the case in a distributed computing paradigm. In the context of distributed self-stabilizing MAS, when agents know the connectivity graph, we may be able to solve the POSG; otherwise  we need to reconsider our game modeling approach. In particular, the connectivity graph in a selfish self-stabilizing system is crucial because even when two agents have similar self-interests, their payoffs and available (guarded) actions still depend on the guards concerning neighbors \dt{don't follow last part}.

In the case of a distributed system, agents may not be aware of the entire connectivity graph, which poses a major problem because regardless of whether the agents are similar or not, their existing payoffs and actions depend on their position in the graph.

\subsection*{POSG on Network Structure}

Self-stabilization of a distributed MAS is a sort of collective intelligence where each agent is choosing actions based on its local knowledge, but eventually, this guarantees global convergence; therefore, local knowledge is a necessary and sufficient condition. In this regard, we expect that an agent knows its exact local connectivity graph at each stage. This particular view of a game, where an agent chooses an action, and then the payoff of each agent is determined by those of its neighbors is very similar to games on networks \cite{galeotti_network_2010}. A network game is a single-stage game where players are connected via a network structure. Any single-stage game in a distributed MAS can be modeled as a network game with incomplete information, where instead of a known 
%network of interactions,\dt{have you introduced interaction?} 
connectivity graph
players are unsure about the network that is in place but have some idea of the number of 
%interactions
connections
 that they will have \cite{menache_network_2011}. The equilibrium concept for this game is Bayesian Nash Equilibrium \cite{harsanyi1967games, Jackson_2008}. Moreover, games in a distributed self-stabilizing MAS are multi-stage (stochastic), and agents need to acquire local observations to estimate local states. In summary, any game in a distributed self-stabilizing system is a series of 
 %different \dt{(?)}
 Bayesian games (i.e., stochastic Bayesian game \cite{albrecht_belief_2016}) that have properties similar to a partially observable stochastic game.

Games on a self-stabilization MAS are not anonymous because agents are connected by a network; however, agents only care about their neighbors' actions. Therefore, given that an agent has no information about the network beyond its locality, it still can play with the agents in its neighborhood but needs to generate beliefs about the locality of agents about whom has incomplete information. An agent’s private knowledge of own locality is interpreted as agent's own type. 

We claim that
 %the local connectivity graph \dt{not sure what a local connectivity graph is}
the neighborhood of an agent $v$
 is enough for $v$ to devise a new set of states $\mathfrak{C}$, as an abstraction of $C$ that can cover all possible available actions and payoffs for every agent in $\ell_v$. Next, we need to provide a conditional distribution over $\mathfrak{C}$ conditioned on local state $\lambda$ and types (i.e., a general description of the state of an agent) of the nearest agents outside the neighborhood. Furthermore, we need to modify (localize) $g_v$ to depend on $\mathfrak{C}$.

Our model for a self-stabilizing MAS that takes accounts for a partially observable environment and incomplete information is $\left<\mathfrak{a}, \ell,\mathfrak{C},\{A_v^\mathfrak{c}\},\Lambda,O,\{\Theta_u\},\mathcal{P},\mathcal{B},\lambda^0,\{g_v\}\right>$, where 
\begin{itemize}
	\item $\mathfrak{a}$ is the agent that models the game,
	\item $\ell$ is the set of agents including $\mathfrak{a}$ and its one-hop and two-hop neighborhoods, where $\ell^*\subset \ell$ includes any agent for which $\mathfrak{a}$ doesn't have its complete information,
	\item $\mathfrak{C}$ is a finite set of states,
	\item $A_v^\mathfrak{c}$ is a finite set of actions available to agent $v$ in state $\mathfrak{c}$, where $v \in \ell$ and $\mathfrak{c} \in \mathfrak{C}$,
	\item $\Lambda$ is the finite set of local states specific to $\mathfrak{a}$,% \dt{is this specific to a given node?  Should it be $\Lambda_v$?}%, where $\lambda^{\mathfrak{c}}$ denotes a distribution on $\Lambda$ for state $\mathfrak{c} \in \mathfrak{C}$ and local state $\lambda\in \Lambda$, i.e., $\Pr(\lambda\mid \mathfrak{c})$%. In the special case that $\lambda \subset \mathfrak{c}$, we have $\Lambda(\mathfrak{c})=\lambda$. We show the state of network beyond the locality with $\mathfrak{c}-\lambda$.
	\item $g_v: \mathfrak{C} \rightarrow \mathbb{R}$ is the gain function of agent $v \in \ell$,
	\item $O$ is a finite set of observations, where an observation $o \in O$ depends on the new local state $\lambda' \in \Lambda$ and on the just taken joint actions $\vec{a} \in \prod_{v\in V}A_v^\mathfrak{c}$ with probability $\Pr(o\mid \lambda',\vec{a})$,% $\lambda^{o}$ denotes a distribution on $\Lambda$ for observation $o \in O$, and $o^{\lambda,\vec{a}}$ denotes a distribution on $O$ after taking joint actions $\vec{a}$ and reaching local state $\lambda$%, i.e., $\Pr(o\mid \lambda,\vec{a})$
	\item $\Theta_u$ is a set of types of agent $u \in \ell^*$ and $\Theta \in \prod_{u\in\ell^*}\Theta_u$ is the set of joint types, where $\theta=\left<\theta_1,\dots,\theta_{|\ell^*|}\right>$ denotes a joint type,  %\dt{introduce types earlier and what role they will play. Also what is $\ell^*$}
	\item $\mathcal{P}$ is a set of conditional transition probabilities between local states, where $\mathcal{P}^(\lambda'\mid \lambda, \vec{a})$ denotes the probability of transition from $\lambda$ to $\lambda'$ after joint action $\vec{a}$; $\lambda, \lambda'\in \Lambda$,%. In the special case that $\lambda \subset \mathfrak{c}$, $T(\mathfrak{c'}\mid \mathfrak{c}, a) = \Pr(\mathfrak{c'}-\Lambda(\mathfrak{c'})\mid \mathfrak{c}, a)\Pr(\Lambda(\mathfrak{c'})\mid \lambda,a)$
	\item $\mathcal{B}$ is a conditional probability distribution over the state space $\mathfrak{c}$, where $\mathcal{B}(\mathfrak{c}\mid \lambda,\vec{\theta})$ denotes the conditional probability of state $\mathfrak{c}$ given the current local state $\lambda\in \Lambda$ and joint type $\vec{\theta}\in \Theta$,% i.e., $\Pr(\mathfrak{c}\mid \lambda,\vec{\theta})$%. In the special case that $\lambda \subset \mathfrak{c}$, $\Pr(\mathfrak{c}\mid \lambda,\theta)$ is simply equal to $\Pr(\mathfrak{c}-\lambda\mid \lambda,\theta)$
	\item $\mathfrak{L} \in \Delta(\Lambda)$ is the initial distribution over local states. %\dt{what is $\Delta$?  Also you introduced $\lambda$ as a state earlier but now $\lambda^0$ is a distribution - use different notation}
\end{itemize}

A type $\theta_u \in \Theta_u$ represents a general but necessary information (specific to the problem that the self-stabilizing algorithm solves) about the network sub-graph branched from the agent $u \in \ell^*$, and depends on the history of actions and local states, $h$, with probability $\Pr(\theta_u\mid h^t)$, where $h^t$ is the history at time $t$. Figure \ref{fig:graph} shows an example of $\mathfrak{a}$, $\ell$, $\ell^*$, and $\theta$.% \dt{I am lost, I don't understand what atype is much less why you need it.}
\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{plots/graph.PNG}
	\captionof{figure}{A sample graph which shows the two-hop neighborhood (set $\ell$) of agent $\textbf{a}$  including itself and the agents with the numbering pattern. Any node with the capital letters represents a possible set of agents outside the neighborhood of $\textbf{a}$, which have at least one neighbor (gray nodes) in the neighborhood.}
	\label{fig:graph}
\end{figure}

Given that $\theta$ has the Markov property $\Pr(\theta\mid h)=\Pr(\theta\mid \lambda',\vec{a})$, we have 
\begin{equation}
\Pr(\mathfrak{c'}\mid \lambda,\vec{a})=\sum_{\theta \in \Theta}\sum_{\lambda'\in\Lambda}\mathcal{B}(\mathfrak{c'}\mid \lambda',\theta)\Pr(\theta\mid \lambda',\vec{a})\mathcal{P}(\lambda'\mid \lambda,\vec{a})
\end{equation}

The model can be formulated as a POSG if $\theta$ is Markovian, and
% either of the following is true: no set of actions is state-dependent; or 
the conditional probability $\Pr(\lambda \mid \mathfrak{c})$ and $\theta^0 \in \Delta(\Theta)$ (i.e., the initial distribution over the joint types) is given.
Then, we have

%In the first case, the POSG form of the model is the tuple $\left<\ell,\Lambda,\{A_v\},\{O\},\mathcal{P},\delta,{\lambda^0},\{U_v^\lambda\}\right>$, where
%\begin{equation}
%U_v^\lambda(\vec{a})=\sum_{\mathfrak{c}'\in\mathfrak{C}}\Pr(\mathfrak{c'}\mid \lambda,\vec{a})\big(g_v(\mathfrak{c}')-\sum_{\mathfrak{c}\in\mathfrak{C}}\sum_{\theta \in \Theta}g_v(\mathfrak{c})\mathcal{B}(\mathfrak{c}\mid \lambda,\theta)\big)
%\end{equation}

%In the second case, where $\Pr(\lambda\mid \mathfrak{c})$ and $\theta^0 \in \Delta(\Theta)$ is given, we have 
\begin{align}
\label{x2x1_eq}
\Pr(\mathfrak{c'}\mid \mathfrak{c},\vec{a})&=\sum_{\lambda\in\Lambda}\Pr(\mathfrak{c'}\mid \lambda,\vec{a})\Pr(\lambda\mid \mathfrak{c}) \\
\label{x2x2_eq}
\Pr(o\mid \mathfrak{c'},\vec{a})&=\sum_{\lambda'\in\Lambda}\Pr(o\mid \lambda',\vec{a})\Pr(\lambda'\mid \mathfrak{c'})
\end{align}
and the initial distribution over states is
\begin{equation}
\label{x2x3_eq}
{b^0}(\mathfrak{c})=\sum_{\lambda\in\Lambda}\sum_{\theta \in \Theta}\mathcal{B}(\mathfrak{c}\mid \lambda,\theta)\mathfrak{L}(\lambda)\theta^0(\theta)
\end{equation}

Following \eqref{x2x1_eq}, \eqref{x2x2_eq}, and \eqref{x2x3_eq}, we can use \eqref{x4_eq}, \eqref{xxxx_eq}, and \eqref{xxx_eq} to obtain $U_v^{\mathfrak{c}}(\vec{a})$, $T(\mathfrak{c},o\mid \mathfrak{c}',\vec{a})$, and $\tau(b,\vec{a},o)$ respectively. The resulting POSG will thus be  $\left<\ell,\mathfrak{C},\{A_v^\mathfrak{c}\},O,T,\delta,{b^0},\{U_v^\mathfrak{c}\}\right>$.
 
It is intractable to solve large POSGs. In \cite{horak_solving_2019}, the authors proposed that a viable alternative is for agents to interleave planning and execution by building and solving a smaller approximate game at every stage to generate actions. Another algorithm that uses heuristics to approximate POSGs is proposed in \cite{emery2004approximate,szer2012maa}.

 Suppose each state $\mathfrak{c}$ is associated with exactly one local state $\lambda \in \Lambda$ and let $y \in Y$ denote a description of agents outside the two-hop neighborhood (i.e., $V\setminus \ell$) such that for any configuration $c$  that is abstracted to $\mathfrak{c}$, there is exactly one element of the product of $\Lambda$ and $Y$ that specifies $c$. For example, suppose $\mathfrak{c}$ is defined by a pair $(\lambda,y)$. Then, we can use \eqref{xN7_eq} and \eqref{xN8_eq} to simplify the POSG.
 
 Let $f_1:\mathfrak{C}\rightarrow\Lambda$ with $f_1(\mathfrak{c})=\lambda$ and let $f_2:\mathfrak{C}\rightarrow Y$ with $f_2(\mathfrak{c})=y$. We have
\begin{equation}
\label{xN7_eq}
\mathcal{B}(\mathfrak{c}\mid\lambda,\theta)=\Pr(f_2(\mathfrak{c})\mid \lambda,\theta)
\end{equation}
\begin{equation}
\label{xN8_eq}
\Pr(\mathfrak{c'}\mid \mathfrak{c}, \vec{a}) = \Pr(y'\mid \mathfrak{c}, \vec{a})\mathcal{P}(\lambda'\mid \lambda,\vec{a})
\end{equation}
where $\lambda=f_1(\mathfrak{c})$, $\lambda'=f_1(\mathfrak{c'})$, $y=f_2(\mathfrak{c})$, and $y'=f_2(\mathfrak{c'})$.

%Given that each state is defined by a pair $(\lambda,y)$ such that $\lambda \in \Lambda$ and $y \in Y$, we can use \eqref{xN7_eq} and \eqref{xN8_eq} to simplify the POSG. %\dt{Reduce to what?}

==> tables/TV1.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|}
\cline{2-6}
&\multicolumn{1}{ |c|  }{}&&&&    \\[-2ex]
& unique & mean & min & max & variance \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &&&&    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 1521.00 & 6.57 & 1.00 & 78.00 & 65.87 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 8.00 & 1250.00 & 97.00 & 4868.00 & 2535269.71 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 1405.00 & 7.12 & 1.00 & 109.00 & 111.83 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 1435.00 & 6.97 & 1.00 & 91.00 & 82.55 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 1213.00 & 8.24 & 1.00 & 154.00 & 171.90 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 2.00 & 5000.00 & 2359.00 & 7641.00 & 13949762.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 1.00 & 10000.00 & 10000.00 & 10000.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{1-fault.}
\label{table:rda}
\end{table*}

==> tables/TV2.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|}
\cline{2-5}
&\multicolumn{1}{ |c|  }{}&&&    \\[-2ex]
& mean & min & max & variance \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &&&    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 16.09 & 11.00 & 18.00 & 1.96 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 16.50 & 15.00 & 17.00 & 0.75 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 15.90 & 11.00 & 18.00 & 2.08 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 16.39 & 12.00 & 18.00 & 1.78 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 16.92 & 12.00 & 18.00 & 1.21 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 12.00 & 12.00 & 12.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 16.00 & 16.00 & 16.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{1-fault.}
\label{table:rda}
\end{table*}

==> tables/TV3.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|}
\cline{2-6}
&\multicolumn{1}{ |c|  }{}&&&&    \\[-2ex]
& unique & mean & min & max & variance \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &&&&    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 1975.00 & 5.06 & 1.00 & 75.00 & 39.77 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 796.00 & 12.56 & 1.00 & 873.00 & 2186.84 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 2053.00 & 4.87 & 1.00 & 68.00 & 29.75 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 1740.00 & 5.75 & 1.00 & 114.00 & 75.94 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 1342.00 & 7.45 & 1.00 & 201.00 & 213.24 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 687.00 & 14.56 & 1.00 & 2737.00 & 12999.24 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 1.00 & 10000.00 & 10000.00 & 10000.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{1-fault.}
\label{table:rda}
\end{table*}

==> tables/TV4.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|}
\cline{2-5}
&\multicolumn{1}{ |c|  }{}&&&    \\[-2ex]
& mean & min & max & variance \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &&&    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 15.26 & 6.00 & 18.00 & 3.82 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 14.83 & 8.00 & 18.00 & 2.21 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 15.01 & 6.00 & 18.00 & 4.31 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 15.62 & 6.00 & 18.00 & 3.59 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 16.26 & 6.00 & 18.00 & 1.79 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 8.89 & 6.00 & 18.00 & 10.62 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 16.00 & 16.00 & 16.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{1-fault.}
\label{table:rda}
\end{table*}

==> tables/arch/T.tex <==
\begin{tabular}{lllllll}
& validity & clusters & moves & rounds & aftermath & successes \\ 
\hline 
bMIS & 100 & 6.7 & 3.3 & 2.3 & 0.7 & 0.3 \\ 
tMIS & 100 & 6.7 & 3.8 & 3.3 & 0 & 0 \\ 
pfMIS & 100 & 6.4 & 1 & 1.1 & 0 & 0 \\ 
vtMIS & 100 & 6.5 & 1.5 & 2.3 & 0.5 & 0.2 \\ 
sMIS & 100 & 7.1 & 1 & 1.1 & 0 & 0 \\ 
vpMIS & 100 & 6.7 & 1 & 1.3 & 0 & 0 \\ 
vpMISf & 100 & 6.5 & 1 & 1.2 & 0.2 & 0.1 \\ 
dpMIS & 100 & 6.3 & 3 & 1.6 & 0 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/T2.tex <==
\begin{tabular}{lllllll}
& trialsS1 & successesS1 & rateS1 & trialsS2 & successesS2 & rateS2 \\ 
\hline 
bMIS & 2 & 1 & 0.5 & 10 & 2 & 0.2 \\ 
tMIS & 22 & 12 & 0.54545 & 39 & 23 & 0.58974 \\ 
pfMIS & 2 & 0 & 0 & 10 & 3 & 0.3 \\ 
vtMIS & 2 & 0 & 0 & 10 & 3 & 0.3 \\ 
sMIS & 2 & 0 & 0 & 10 & 3 & 0.3 \\ 
vpMIS & 38 & 24 & 0.63158 & 54 & 31 & 0.57407 \\ 
vpMISf & 2 & 1 & 0.5 & 10 & 3 & 0.3 \\ 
dpMIS & 15 & 0 & 0 & 43 & 0 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/T21.tex <==
\begin{tabular}{lllllll}
& trialsS1 & successesS1 & rateS1 & trialsS2 & successesS2 & rateS2 \\ 
\hline 
vpMIS & 35 & 1 & 0.028571 & 34 & 0 & 0 \\ 
dpMIS & 13 & 0 & 0 & 34 & 0 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/TV1.tex <==
\begin{tabular}{llllll}
& unique & mean & min & max & variance \\ 
\hline 
bMIS & 10 & 1 & 1 & 1 & 0 \\ 
tMIS & 4 & 2.5 & 1 & 6 & 5.6667 \\ 
pfMIS & 10 & 1 & 1 & 1 & 0 \\ 
vtMIS & 9 & 1.1111 & 1 & 2 & 0.11111 \\ 
sMIS & 4 & 2.5 & 1 & 5 & 3.6667 \\ 
vpMIS & 1 & 10 & 10 & 10 & 0 \\ 
vpMISf & 5 & 2 & 1 & 5 & 3 \\ 
dpMIS & 1 & 10 & 10 & 10 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/TV2.tex <==
\begin{tabular}{lllll}
& mean & min & max & variance \\ 
\hline 
bMIS & 6.7 & 5 & 9 & 1.5667 \\ 
tMIS & 6.4 & 4 & 7 & 0.93333 \\ 
pfMIS & 7.6 & 5 & 9 & 2.4889 \\ 
vtMIS & 7.5 & 5 & 9 & 1.3889 \\ 
sMIS & 8.6 & 7 & 9 & 0.71111 \\ 
vpMIS & 6 & 6 & 6 & 0 \\ 
vpMISf & 6.2 & 4 & 7 & 1.5111 \\ 
dpMIS & 9 & 9 & 9 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/TV3.tex <==
\begin{tabular}{llllll}
& unique & mean & min & max & variance \\ 
\hline 
bMIS & 10 & 1 & 1 & 1 & 0 \\ 
tMIS & 10 & 1 & 1 & 1 & 0 \\ 
pfMIS & 10 & 1 & 1 & 1 & 0 \\ 
vtMIS & 10 & 1 & 1 & 1 & 0 \\ 
sMIS & 10 & 1 & 1 & 1 & 0 \\ 
vpMIS & 10 & 1 & 1 & 1 & 0 \\ 
vpMISf & 10 & 1 & 1 & 1 & 0 \\ 
dpMIS & 10 & 1 & 1 & 1 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch/TV4.tex <==
\begin{tabular}{lllll}
& mean & min & max & variance \\ 
\hline 
bMIS & 7.2 & 5 & 9 & 1.2889 \\ 
tMIS & 6.9 & 5 & 8 & 0.98889 \\ 
pfMIS & 6.7 & 5 & 8 & 1.3444 \\ 
vtMIS & 7 & 6 & 8 & 0.88889 \\ 
sMIS & 7.2 & 6 & 8 & 0.62222 \\ 
vpMIS & 7.1 & 6 & 8 & 0.54444 \\ 
vpMISf & 6.6 & 5 & 8 & 0.93333 \\ 
dpMIS & 6.8 & 5 & 8 & 1.0667 \\ 
\hline 
\end{tabular}

==> tables/arch2/Availability.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ cc|c|c|c|c|c|c|c|c|  }
\cline{3-9}
&&\multicolumn{7}{ |c| }{}\\[-1.9ex]
&&\multicolumn{7}{ |c| }{Availability}\\[0.3ex]
\cline{2-9}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} &  {$vp$MIS} &  {$dp$MIS}\\[0.3ex]
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.89 & 0.89 & 0.90 & 0.86 & 0.87 & 0.90 & 0.81 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.83 & 0.75 & 0.90 & 0.76 & 0.87 & 0.51 & 0.83 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.62 & 0.89 & 0.62 & 0.87 & 0.87 & 0.91 & 0.81 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.17 & 0.56 & 0.61 & 0.75 & 0.87 & 0.48 & 0.82 \\[0.3ex] 
\hline 
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.91 & 0.91 & 0.93 & 0.88 & 0.86 & 0.93 & 0.92 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.83 & 0.79 & 0.92 & 0.56 & 0.86 & 0.57 & 0.92 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.51 & 0.91 & 0.49 & 0.87 & 0.86 & 0.94 & 0.91 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.02 & 0.44 & 0.52 & 0.56 & 0.86 & 0.56 & 0.92 \\[0.3ex] 
\hline 
\end{tabular}
\caption{Impact of deviation type on availability in a (top) sparse network where \# of agents is 100 and average degree is 4, and (bottom) dense network where \# of agents is 100 and average degree is 20.}
\label{table:rda}
\end{table*}

==> tables/arch2/NumberOfDeviations.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ cc|c|c|c|c|c|c|c|c|  }
\cline{3-9}
&&\multicolumn{7}{ |c| }{}\\[-1.9ex]
&&\multicolumn{7}{ |c| }{Average \# of Deviations}\\[0.3ex]
\cline{2-9}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} &  {$vp$MIS} &  {$dp$MIS}\\[0.3ex]
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 451.49 & 267.25 & 0.00 & 423.11 & 0.00 & 487.78 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 2995.39 & 561.15 & 2949.39 & 0.00 & 0.00 & 0.00 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 6690.30 & 2202.98 & 3077.22 & 447.70 & 0.00 & 546.51 & 0.00 \\[0.3ex] 
\hline 
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 476.79 & 121.71 & 0.00 & 278.18 & 0.00 & 119.22 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 4761.43 & 242.91 & 5109.74 & 0.00 & 0.00 & 0.00 & 0.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 9654.00 & 2498.55 & 4766.84 & 283.59 & 0.00 & 124.95 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{Impact of deviation type on average \# of deviations in a (top) sparse network where \# of agents is 100 and average degree is 4, and (bottom) dense network where \# of agents is 100 and average degree is 20.}
\label{table:rda}
\end{table*}

==> tables/arch2/Reliability.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ cc|c|c|c|c|c|c|c|c|  }
\cline{3-9}
&&\multicolumn{7}{ |c| }{}\\[-1.9ex]
&&\multicolumn{7}{ |c| }{Reliability}\\[0.3ex]
\cline{2-9}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} &  {$vp$MIS} &  {$dp$MIS}\\[0.3ex]
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.00 & 0.05 & 0.00 & 1.00 & 1.00 & 1.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 \\[0.3ex] 
\hline 
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  & &  \\[-2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.00 & 0.00 & 1.00 & 0.00 & 1.00 & 0.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.00 & 0.58 & 0.00 & 1.00 & 1.00 & 1.00 & 1.00 \\[0.8ex] 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.00 & 0.00 & 0.00 & 0.00 & 1.00 & 0.00 & 1.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{Impact of deviation type on reliability in a (top) sparse network where \# of agents is 100 and average degree is 4, and (bottom) dense network where \# of agents is 100 and average degree is 20.}
\label{table:rda}
\end{table*}

==> tables/arch2/T.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c| }
\cline{2-5}
&\multicolumn{1}{ |c|  }{}&  &    &    \\[-2ex]
& moves & rounds & aftermath & successes \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &    &    &    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 1.00 & 1.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 42.00 & 4.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 1.00 & 2.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 1.00 & 1.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 1.00 & 1.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 1.00 & 1.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 9.00 & 2.00 & 0.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{1-fault.}
\label{table:rda}
\end{table*}

==> tables/arch2/T2.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|c| }
\cline{2-7}
&\multicolumn{3}{ |c| }{} &\multicolumn{3}{ |c| }{}\\[-1.9ex]
&\multicolumn{3}{ |c| }{Scenario 1} &\multicolumn{3}{ |c| }{Scenario 2}\\ 
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2ex]
& \# of trials & \# of successes & rate &  \# of trials & \# of successes & rate \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &    &    &    & &  \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 0.00 & 0.00 & NaN & 3.00 & 1.00 & 0.33 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 1.00 & 1.00 & 1.00 & 4.00 & 2.00 & 0.50 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 0.00 & 0.00 & NaN & 3.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 0.00 & 0.00 & NaN & 3.00 & 1.00 & 0.33 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 0.00 & 0.00 & NaN & 3.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 1.00 & 1.00 & 1.00 & 5.00 & 3.00 & 0.60 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 0.00 & 0.00 & NaN & 2.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS\^*}& 0.00 & 0.00 & NaN & 0.00 & 0.00 & NaN \\[0.3ex] 
\hline 
\end{tabular}
\caption{ Dead-ends Case 2.}
\label{table:rda}
\end{table*}

==> tables/arch2/T21.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|c| }
\cline{2-7}
&\multicolumn{3}{ |c| }{} &\multicolumn{3}{ |c| }{}\\[-1.9ex]
&\multicolumn{3}{ |c| }{Scenario 1} &\multicolumn{3}{ |c| }{Scenario 2}\\ 
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2ex]
& \# of trials & \# of successes & rate &  \# of trials & \# of successes & rate \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &    &    &    & &  \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 0.00 & 0.00 & NaN & 4.00 & 1.00 & 0.25 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 0.00 & 0.00 & NaN & 3.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 1.00 & 1.00 & 1.00 & 4.00 & 2.00 & 0.50 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 0.00 & 0.00 & NaN & 4.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 2.00 & 1.00 & 0.50 & 5.00 & 1.00 & 0.20 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 0.00 & 0.00 & NaN & 3.00 & 0.00 & 0.00 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 3.00 & 0.00 & 0.00 & 3.00 & 0.00 & 0.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{ Dead-end Case I}
\label{table:rda}
\end{table*}

==> tables/arch2/TV1.tex <==
\begin{tabular}{llllll}
& unique & mean & min & max & variance \\ 
\hline 
bMIS & 47 & 212.766 & 17 & 773 & 27064.3136 \\ 
tMIS & 1 & 10000 & 10000 & 10000 & 0 \\ 
pfMIS & 47 & 212.766 & 16 & 753 & 33177.0093 \\ 
vtMIS & 47 & 212.766 & 8 & 800 & 31101.6614 \\ 
dtMIS & 95 & 105.2632 & 2 & 785 & 24829.196 \\ 
vpMIS & 1 & 10000 & 10000 & 10000 & 0 \\ 
dpMIS & 1 & 10000 & 10000 & 10000 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch2/TV2.tex <==
\begin{tabular}{lllll}
& mean & min & max & variance \\ 
\hline 
bMIS & 6.728 & 4 & 7 & 0.24304 \\ 
tMIS & 6 & 6 & 6 & 0 \\ 
pfMIS & 6.6611 & 4 & 7 & 0.28668 \\ 
vtMIS & 6.7934 & 4 & 7 & 0.18233 \\ 
dtMIS & 6.8373 & 4 & 7 & 0.15004 \\ 
vpMIS & 6 & 6 & 6 & 0 \\ 
dpMIS & 6 & 6 & 6 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch2/TV3.tex <==
\begin{tabular}{llllll}
& unique & mean & min & max & variance \\ 
\hline 
bMIS & 149 & 67.1141 & 7 & 245 & 2075.7909 \\ 
tMIS & 133 & 75.188 & 1 & 1155 & 23550.1992 \\ 
pfMIS & 149 & 67.1141 & 13 & 201 & 1469.4937 \\ 
vtMIS & 149 & 67.1141 & 11 & 272 & 2993.4531 \\ 
dtMIS & 149 & 67.1141 & 5 & 390 & 6225.2504 \\ 
vpMIS & 137 & 72.9927 & 1 & 1639 & 33052.5955 \\ 
dpMIS & 1 & 10000 & 10000 & 10000 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch2/TV4.tex <==
\begin{tabular}{lllll}
& mean & min & max & variance \\ 
\hline 
bMIS & 5.8744 & 4 & 7 & 0.56348 \\ 
tMIS & 5.2764 & 4 & 7 & 0.23243 \\ 
pfMIS & 5.8043 & 4 & 7 & 0.56866 \\ 
vtMIS & 5.9641 & 4 & 7 & 0.55367 \\ 
dtMIS & 6.1629 & 4 & 7 & 0.52202 \\ 
vpMIS & 5.2576 & 4 & 7 & 0.31747 \\ 
dpMIS & 5 & 5 & 5 & 0 \\ 
\hline 
\end{tabular}

==> tables/arch2/TV5.tex <==
\begin{table*}[h!]
\centering
\begin{tabular}{ c|c|c|c|c|c|c|}
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&&&&&    \\[-2ex]
& uniqueConfs1 & avgConfRepeat1 & avgNClstrs1 & uConfs & avgCnfRep & avgNCls \\ 
\hline
\multicolumn{1}{ |c|  }{}&  &&&&&    \\[-2ex]
\multicolumn{1}{ |c| }{$b$MIS}& 98.00 & 1.02 & 13.15 & 95.00 & 1.05 & 16.07 \\[0.6ex] 
\multicolumn{1}{ |c| }{$t$MIS}& 7.00 & 14.29 & 11.81 & 90.00 & 1.11 & 14.20 \\[0.6ex] 
\multicolumn{1}{ |c| }{$pf$MIS}& 99.00 & 1.01 & 13.21 & 94.00 & 1.06 & 15.69 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vt$MIS}& 94.00 & 1.06 & 13.97 & 91.00 & 1.10 & 16.60 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dt$MIS}& 94.00 & 1.06 & 14.05 & 90.00 & 1.11 & 17.15 \\[0.6ex] 
\multicolumn{1}{ |c| }{$vp$MIS}& 10.00 & 10.00 & 10.35 & 50.00 & 2.00 & 10.70 \\[0.6ex] 
\multicolumn{1}{ |c| }{$dp$MIS}& 1.00 & 100.00 & 14.00 & 1.00 & 100.00 & 13.00 \\[0.3ex] 
\hline 
\end{tabular}
\caption{outcome.}
\label{table:rda}
\end{table*}

==> tables/arch3/Availability.tex <==

\scalebox{0.885}{\begin{tabular}{ cc|c|c|c|c|c|c|  }
\cline{3-7}
&&\multicolumn{5}{ |c| }{}\\[-2.2ex]
&&\multicolumn{5}{ |c| }{Availability}\\
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.2ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} \\
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.91 & 0.89 & 0.92 & 0.89 & 0.89  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.84 & 0.77 & 0.92 & 0.78 & 0.89  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.62 & 0.90 & 0.62 & 0.89 & 0.89  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.23 & 0.59 & 0.62 & 0.78 & 0.89  \\[0.1ex] 
\hline 
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.93 & 0.90 & 0.94 & 0.89 & 0.87  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.84 & 0.83 & 0.94 & 0.55 & 0.87  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.52 & 0.87 & 0.52 & 0.89 & 0.87  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.02 & 0.35 & 0.51 & 0.55 & 0.87  \\[0.1ex] 
\hline 
\label{table:aa}
\end{tabular}}

==> tables/arch3/NumberOfDeviations.tex <==

\scalebox{0.885}{\begin{tabular}{ cc|c@{\hspace{0.47em}}|@{\hspace{0.47em}}c@{\hspace{0.47em}}|@{\hspace{0.47em}}c@{\hspace{0.47em}}|c|c|c|  }
\cline{3-7}
&&\multicolumn{5}{ |c| }{}\\[-2.2ex]
&&\multicolumn{5}{ |c| }{Average \# of Deviations}\\
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2.2ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} \\
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2.2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 451.6 & 267.0 & 0.0 & 404.7 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 3166.5 & 432.7 & 2929.9 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 6471.7 & 1937.1 & 2957.0 & 400.0 & 0.0  \\[0.1ex] 
\hline 
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &    \\[-2.2ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 450.1 & 150.6 & 0.0 & 275.5 & 0.0  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 4516.5 & 351.9 & 4792.6 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 9318.1 & 3430.9 & 4855.1 & 278.8 & 0.0  \\[0.1ex] 
\hline 
\label{table:dr}
\end{tabular}}


==> tables/arch3/Reliability.tex <==

\scalebox{1}{\begin{tabular}{ cc|c|c|c|c|c|c|  }
\cline{3-7}
&&\multicolumn{5}{ |c| }{}\\[-2.5ex]
&&\multicolumn{5}{ |c| }{Reliability}\\
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &    \\[-2.4ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS}\\
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.00 & 0.00 & 1.00 & 0.00 & 1.00 \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.00 & 0.05 & 0.00 & 1.00 & 1.00 \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
\hline 
&&\multicolumn{5}{ |c| }{}\\[-2.7ex]
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.00 & 0.00 & 1.00 & 0.00 & 1.00 \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.00 & 0.65 & 0.00 & 1.00 & 1.00  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.00 & 0.00 & 0.00 & 0.00 & 1.00 \\
\hline 
&&\multicolumn{5}{ |c| }{}\\[-2.5ex]
\cline{3-7}
&&\multicolumn{5}{ |c| }{}\\[-2.5ex]
&&\multicolumn{5}{ |c| }{Average \# of Deviations}\\
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2.4ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} \\
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &  \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 451.6 & 267.0 & 0.0 & 404.7 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 3166.5 & 432.7 & 2929.9 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 6471.7 & 1937.1 & 2957.0 & 400.0 & 0.0  \\
\hline 
&&\multicolumn{5}{ |c| }{}\\[-2.7ex]
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &    \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.0 & 0.0 & 0.0 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 450.1 & 150.6 & 0.0 & 275.5 & 0.0  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 4516.5 & 351.9 & 4792.6 & 0.0 & 0.0  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 9318.1 & 3430.9 & 4855.1 & 278.8 & 0.0  \\
\hline 
&&\multicolumn{5}{ |c| }{}\\[-2.5ex]
\cline{3-7}
&&\multicolumn{5}{ |c| }{}\\[-2.5ex]
&&\multicolumn{5}{ |c| }{Availability}\\
\cline{2-7}
&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.4ex]
&\multicolumn{1}{ |c| }{Dev. type}& {$b$MIS}&    {$t$MIS}&    {$pf$MIS}&    {$vt$MIS} &  {$dt$MIS} \\
\hline
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Sparse}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.91 & 0.89 & 0.92 & 0.89 & 0.89  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.84 & 0.77 & 0.92 & 0.78 & 0.89  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.62 & 0.90 & 0.62 & 0.89 & 0.89  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.23 & 0.59 & 0.62 & 0.78 & 0.89  \\
\hline 
&&\multicolumn{5}{ |c| }{}\\[-2.7ex]
\hline 
\multicolumn{1}{ |c  }{\multirow{5}{*}{\rotatebox[origin=c]{90}{Dense}}}&\multicolumn{1}{ |c|  }{}&  &    &    &    &   \\[-2.5ex]
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{No Deviation}& 0.93 & 0.90 & 0.94 & 0.89 & 0.87  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Perturbation}& 0.84 & 0.83 & 0.94 & 0.55 & 0.87  \\
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Violation}& 0.52 & 0.87 & 0.52 & 0.89 & 0.87  \\ 
\multicolumn{1}{ |c  }{}&\multicolumn{1}{ |c| }{Deflection}& 0.02 & 0.35 & 0.51 & 0.55 & 0.87  \\
\hline 
\label{table:rr}
\end{tabular}}
